Differentiable Likelihoods for Fast Inversion of 'Likelihood-Free' Dynamical Systems

Likelihood-free (a.k.a. simulation-based) inference problems are inverse problems with expensive, or intractable, forward models. ODE inverse problems are commonly treated as likelihood-free, as their forward map has to be numerically approximated by an ODE solver. This, however, is not a fundamental constraint but just a lack of functionality in classic ODE solvers, which do not return a likelihood but a point estimate. To address this shortcoming, we employ Gaussian ODE filtering (a probabilistic numerical method for ODEs) to construct a local Gaussian approximation to the likelihood. This approximation yields tractable estimators for the gradient and Hessian of the (log-)likelihood. Insertion of these estimators into existing gradient-based optimization and sampling methods engenders new solvers for ODE inverse problems. We demonstrate that these methods outperform standard likelihood-free approaches on three benchmark-systems.

==> pgfplots/TEX_lv_opt.tex <==
% This file was created by tikzplotlib v0.9.0.
\begin{tikzpicture}[trim axis left,trim axis right,baseline]

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{1,0.498039215686275,0.0549019607843137}
\definecolor{color2}{rgb}{0.172549019607843,0.627450980392157,0.172549019607843}

% \begin{groupplot}[group style={group size=2 by 1}]
\begin{groupplot}[group style={group size=1 by 1}]

\nextgroupplot[
width=\figwidth,
height=\figheight,
scale only axis,
% width=0.3\textwidth,
legend style={at={(0,0)}, xshift=0.15cm, yshift=0.05cm, anchor=south west },
ymode=log,
ylabel={Neg. log-likelihood},
% title = {\bf Optimization}
]
\addplot+
table {%
0 1393098.95998807
1 1393098.95998807
2 1365859.80514612
3 1365859.80514612
4 1365859.80514612
5 1365859.80514612
6 1365859.80514612
7 1352070.20091395
8 1352070.20091395
9 1352070.20091395
10 1352070.20091395
11 1311388.26151442
12 1311388.26151442
13 1236501.54594476
14 1236501.54594476
15 1236501.54594476
16 1185368.71247196
17 1185368.71247196
18 1185368.71247196
19 1185368.71247196
20 1185368.71247196
21 1082060.50200496
22 1082060.50200496
23 1082060.50200496
24 1082060.50200496
25 1082060.50200496
26 1082060.50200496
27 1049762.52403809
28 952490.329864678
29 952490.329864678
30 952490.329864678
31 952490.329864678
32 832550.814325873
33 779712.756222619
34 776359.357103089
35 722430.922418072
36 722430.922418072
37 645134.153492063
38 578699.92921578
39 492371.988754658
40 381922.382748681
41 381922.382748681
42 381922.382748681
43 355413.945745475
44 355413.945745475
45 355413.945745475
46 355413.945745475
47 355413.945745475
48 355413.945745475
49 355413.945745475
};
\addlegendentry{RS}
\addplot+
table {%
0 1393098.95998807
1 1090605.53183751
2 821637.586886575
3 593264.615703072
4 421713.758066416
5 328239.616831898
6 331424.596552061
7 416450.097049457
8 457093.064699312
9 236721.769535925
10 134257.987476327
11 156029.929407882
12 65755.3677595245
13 40390.9268152136
14 57273.5929519011
15 53193.6242778977
16 18673.2210106684
17 9209.18171685116
18 8380.07006718789
19 6717.00296067827
20 10738.0992503794
21 12535.6434538686
22 8016.68885952329
23 3954.7741086071
24 3132.78676607872
25 3802.55662494184
26 5247.47520442604
27 6148.5641834069
28 5596.1063787733
29 4496.34190684225
30 3937.7794651198
31 4052.46527765143
32 4510.33579995626
33 4869.96062804102
34 4854.21108070214
35 4582.53358286371
36 4353.89513763679
37 4320.07867144746
38 4433.98696297984
39 4558.62014549748
40 4590.00336552147
41 4529.02251856823
42 4450.0561033425
43 4416.24227936395
44 4434.56667458476
45 4470.4106088126
46 4487.04158784429
47 4474.30875874768
48 4448.20305647906
49 4429.80745202906
};
\addlegendentry{GD}
\addplot+
table {%
0 1393098.95998807
1 1085013.96608212
2 833645.135401544
3 615009.459950509
4 433326.70872668
5 295122.861999796
6 212949.009719144
7 152289.640306393
8 82940.6641475305
9 63679.5966834178
10 51458.9908232228
11 42870.536941719
12 35373.7587424317
13 28139.6168890103
14 21217.2703160641
15 15012.6064117364
16 9924.01185339072
17 6125.77981277611
18 3534.92430245974
19 1908.05625525718
20 961.907919390796
21 451.106925527424
22 195.891061977816
23 79.0284908345459
24 30.9139241152886
25 13.6745520050523
26 8.53893470132973
27 7.21208377866428
28 6.59538867416741
29 5.8582122167199
30 4.97926672375324
31 4.11516270051029
32 3.38422155708475
33 2.82943049459369
34 2.44060504230154
35 2.18393996260732
36 2.02227273891673
37 1.92467370829928
38 1.86882095238484
39 1.83986082721177
40 1.82824403745247
41 1.82777341098256
42 1.83425351029056
43 1.84470434915806
44 1.85695848119736
45 1.86946486014208
46 1.88117890037196
47 1.89147570394087
48 1.90006369851997
49 1.90689735173486
};
\addlegendentry{NWT}
\end{groupplot}

\end{tikzpicture}


% \nextgroupplot[
% axis line style={white!80!black},
% log basis y={10},
% tick align=outside,
% tick pos=left,
% title={Distance to true parameter},
% x grid style={white!80!black},
% xmajorgrids,
% xmin=-2.45, xmax=51.45,
% xtick style={color=white!15!black},
% y grid style={white!80!black},
% ymajorgrids,
% ymin=0.00106073763964196, ymax=4.11487678045554,
% ymode=log,
% ytick style={color=white!15!black},
% ytick={0.0001,0.001,0.01,0.1,1,10,100},
% yticklabels={\(\displaystyle {10^{-4}}\),\(\displaystyle {10^{-3}}\),\(\displaystyle {10^{-2}}\),\(\displaystyle {10^{-1}}\),\(\displaystyle {10^{0}}\),\(\displaystyle {10^{1}}\),\(\displaystyle {10^{2}}\)}
% ]
% \addplot [ultra thick, color0]
% table {%
% 0 1.14017542509914
% 1 1.14017542509914
% 2 1.07653319681145
% 3 1.07653319681145
% 4 1.07653319681145
% 5 1.07653319681145
% 6 1.07653319681145
% 7 1.10498440528307
% 8 1.10498440528307
% 9 1.10498440528307
% 10 1.10498440528307
% 11 1.03143801002773
% 12 1.03143801002773
% 13 0.952426837335556
% 14 0.952426837335556
% 15 0.952426837335556
% 16 0.879504877170528
% 17 0.879504877170528
% 18 0.879504877170528
% 19 0.879504877170528
% 20 0.879504877170528
% 21 0.792622914543451
% 22 0.792622914543451
% 23 0.792622914543451
% 24 0.792622914543451
% 25 0.792622914543451
% 26 0.792622914543451
% 27 0.78892087553874
% 28 0.731269806388593
% 29 0.731269806388593
% 30 0.731269806388593
% 31 0.731269806388593
% 32 0.658215058981417
% 33 0.625517784427277
% 34 0.627324586931649
% 35 0.625894936609278
% 36 0.625894936609278
% 37 0.552986753194924
% 38 0.544289147143617
% 39 0.473742745334361
% 40 0.401152922904796
% 41 0.401152922904796
% 42 0.401152922904796
% 43 0.389379622300786
% 44 0.389379622300786
% 45 0.389379622300786
% 46 0.389379622300786
% 47 0.389379622300786
% 48 0.389379622300786
% 49 0.389379622300786
% };
% \addplot [ultra thick, color1]
% table {%
% 0 1.14017542509914
% 1 0.972534525116298
% 2 0.840853224962363
% 3 0.754481586621778
% 4 0.711678395246213
% 5 0.69521937631633
% 6 0.675966298883208
% 7 0.621123697662269
% 8 0.507963354236103
% 9 0.377557538563487
% 10 0.345498990605347
% 11 0.245874691560426
% 12 0.229572706541314
% 13 0.28160957158844
% 14 0.312105684301101
% 15 0.30523141239397
% 16 0.281827281738267
% 17 0.252803350075906
% 18 0.232779224058443
% 19 0.24254180590126
% 20 0.260362266222557
% 21 0.267714331808638
% 22 0.263823129739471
% 23 0.25477017811667
% 24 0.247866902593619
% 25 0.24815238615114
% 26 0.252999159380693
% 27 0.256724703872284
% 28 0.256856632335079
% 29 0.254458580527256
% 30 0.252016222928375
% 31 0.251362300036042
% 32 0.252382464372475
% 33 0.253648063440012
% 34 0.254038072626329
% 35 0.253489530005667
% 36 0.252662694487828
% 37 0.252219396510996
% 38 0.252317790712189
% 39 0.252642532121938
% 40 0.25280734805163
% 41 0.252678469766196
% 42 0.252390764008121
% 43 0.252156584055668
% 44 0.252078509915379
% 45 0.252105360685116
% 46 0.252121846374372
% 47 0.252058774802065
% 48 0.251930912178281
% 49 0.251797985719012
% };
% \addplot [ultra thick, color2]
% table {%
% 0 1.14017542509914
% 1 1.18336386613828
% 2 1.49392570244984
% 3 1.71473150104136
% 4 2.22857638364891
% 5 2.82638869205517
% 6 2.25296766652401
% 7 0.655897287756813
% 8 0.362919883910724
% 9 0.442537022314815
% 10 0.520580550652745
% 11 0.550458232140984
% 12 0.538114710698247
% 13 0.494223022226252
% 14 0.430681226183816
% 15 0.358516977023748
% 16 0.286503921725002
% 17 0.220546624027821
% 18 0.163802612337358
% 19 0.117291932700225
% 20 0.0806516346360732
% 21 0.0527820614365598
% 22 0.032291999422822
% 23 0.0177618951550297
% 24 0.00788246296720637
% 25 0.00154430446731801
% 26 0.00236675313237788
% 27 0.00439170615629489
% 28 0.00523958270438084
% 29 0.00534903573919486
% 30 0.00504305881632753
% 31 0.00454522587858311
% 32 0.00400088202633356
% 33 0.00349628165834663
% 34 0.00307491421788762
% 35 0.00275111611235615
% 36 0.00252125279037389
% 37 0.00237247289113385
% 38 0.00228876914472399
% 39 0.00225439393467135
% 40 0.0022553229158506
% 41 0.00227970339723185
% 42 0.00231792839554834
% 43 0.00236257694572966
% 44 0.00240825668641381
% 45 0.00245135364703694
% 46 0.00248971788558575
% 47 0.00252232779887498
% 48 0.00254897158395659
% 49 0.00256997107921563
% };


==> pgfplots/TEX_pst_opt.tex <==
% This file was created by tikzplotlib v0.9.0.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{1,0.498039215686275,0.0549019607843137}
\definecolor{color2}{rgb}{0.172549019607843,0.627450980392157,0.172549019607843}

\begin{groupplot}[group style={group size=1 by 1}]
\nextgroupplot[
legend style={at={(0,0)}, xshift=0.15cm, yshift=0.05cm, anchor=south west },
ymode=log,
xlabel={Iterations $i$},
ylabel={Neg. log-likelihood},
]
\addplot+[mark repeat=5]
table {%
0 240.383424498765
1 237.625860129818
2 235.7065019453
3 234.716584312435
4 233.678774767295
5 232.766717262208
6 232.766717262208
7 232.766717262208
8 232.766717262208
9 232.04207370029
10 232.04207370029
11 232.04207370029
12 232.04207370029
13 232.04207370029
14 231.580293371392
15 231.580293371392
16 231.580293371392
17 231.450521542371
18 231.450521542371
19 230.667353146762
20 230.667353146762
21 230.510274817651
22 230.510274817651
23 230.510274817651
24 230.510274817651
25 230.510274817651
26 230.510274817651
27 230.510274817651
28 228.165885884313
29 226.02069677406
30 225.962509349262
31 225.962509349262
32 225.962509349262
33 225.962509349262
34 223.112072065753
35 221.362874798428
36 221.362874798428
37 221.362874798428
38 221.362874798428
39 221.362874798428
40 221.362874798428
41 221.362874798428
42 221.362874798428
43 221.362874798428
44 221.362874798428
45 219.989309983442
46 219.989309983442
47 219.989309983442
48 219.989309983442
49 219.989309983442
50 219.989309983442
51 219.555841955012
52 219.555841955012
53 217.704712791302
54 217.704712791302
55 217.704712791302
56 216.868570113613
57 216.851763465366
58 216.851763465366
59 216.851763465366
60 214.544714847068
61 214.544714847068
62 214.544714847068
63 214.402577320795
64 214.402577320795
65 214.402577320795
66 214.402577320795
67 213.989232107968
68 213.451040581752
69 213.451040581752
70 213.337411394801
71 213.337411394801
72 210.693285082079
73 210.693285082079
74 210.693285082079
75 210.693285082079
76 210.061889425643
77 210.061889425643
78 210.061889425643
79 208.172634196946
80 208.172634196946
81 207.624202237843
82 207.624202237843
83 207.624202237843
84 207.624202237843
85 207.624202237843
86 207.624202237843
87 205.300574505195
88 203.994650781784
89 203.994650781784
90 203.994650781784
91 203.994650781784
92 203.994650781784
93 203.994650781784
94 203.994650781784
95 203.994650781784
96 203.994650781784
97 203.994650781784
98 203.994650781784
99 203.994650781784
100 203.994650781784
101 202.045772932768
102 202.045772932768
103 202.045772932768
104 200.330451117623
105 200.330451117623
106 200.330451117623
107 199.721490107661
108 198.724334702652
109 198.280234515459
110 197.39539351962
111 195.716214553799
112 195.520945853256
113 194.360953231276
114 194.360953231276
115 193.262361780119
116 193.262361780119
117 193.262361780119
118 193.262361780119
119 193.262361780119
120 193.262361780119
121 193.262361780119
122 193.262361780119
123 193.262361780119
124 193.0894586541
125 193.0894586541
126 192.344648783183
127 189.976443064383
128 187.940470611681
129 186.339376769966
130 186.339376769966
131 186.339376769966
132 186.339376769966
133 185.106480418928
134 184.085614252136
135 182.41786431541
136 182.41786431541
137 182.41786431541
138 181.397733411067
139 179.998195083661
140 179.998195083661
141 179.998195083661
142 179.998195083661
143 177.761331163392
144 177.761331163392
145 177.761331163392
146 177.761331163392
147 177.761331163392
148 177.761331163392
149 177.761331163392
};
\addlegendentry{RS}
\addplot+[mark repeat=5]
table {%
0 240.383424498765
1 232.258459922016
2 227.400836338774
3 225.165550387386
4 222.928956658394
5 220.59044621777
6 218.279363486851
7 215.986328460932
8 213.712779437374
9 211.459204882
10 209.226135491458
11 207.014062791032
12 204.823441653218
13 202.654686689242
14 200.508169088607
15 198.384213499474
16 196.283095014828
17 194.205036303252
18 192.150204927349
19 190.118710894886
20 188.110604489263
21 186.125874426679
22 184.164446387354
23 182.226181967133
24 180.310878093747
25 178.418266948792
26 176.548016432058
27 174.699731199211
28 172.872954296924
29 171.067169411518
30 169.281803738042
31 167.51623146664
32 165.769777872255
33 164.041723982418
34 162.331311786308
35 160.637749936873
36 158.960219886732
37 157.297882388394
38 155.649884280178
39 154.01536547156
40 152.393466035753
41 150.783333313379
42 149.184128929317
43 147.595035625321
44 146.015263813829
45 144.444057763417
46 142.88070133359
47 141.324523185639
48 139.77490140704
49 138.231267498835
50 136.693109688332
51 135.159975542831
52 133.631473873575
53 132.107275932275
54 130.587115915051
55 129.070790800146
56 127.558159555992
57 126.049141764988
58 124.543715715506
59 123.041916020115
60 121.543830821787
61 120.049598651994
62 118.559405005162
63 117.073478693112
64 115.592088041021
65 114.115536983292
66 112.644161113692
67 111.178323739445
68 109.718411983837
69 108.264832976445
70 106.818010164596
71 105.378379774151
72 103.946387442353
73 102.522485040447
74 101.107127698985
75 99.7007710444518
76 98.3038686518954
77 96.9168697148485
78 95.5402169308121
79 94.1743445980685
80 92.8196769174914
81 91.476626491343
82 90.1455930097482
83 88.8269621145765
84 87.5211044298131
85 86.2283747471149
86 84.9491113550969
87 83.6836355009383
88 82.4322509730989
89 81.1952437942748
90 79.9728820141575
91 78.7654155920715
92 77.5730763601416
93 76.3960780582312
94 75.2346164325279
95 74.0888693902708
96 72.9589972037368
97 71.8451427572098
98 70.7474318312369
99 69.6659734190312
100 68.6008600704022
101 67.5521682590856
102 66.5199587697942
103 65.5042771017267
104 64.5051538856554
105 63.5226053120508
106 62.5566335680178
107 61.6072272810875
108 60.6743619681636
109 59.7580004881293
110 58.8580934968182
111 57.9745799032158
112 57.1073873258993
113 56.2564325488489
114 55.421621975867
115 54.6028520829294
116 53.8000098678675
117 53.0129732968406
118 52.2416117471098
119 51.4857864456642
120 50.7453509032846
121 50.0201513436563
122 49.3100271271647
123 48.6148111690229
124 47.9343303513969
125 47.2684059292033
126 46.6168539292639
127 45.9794855425109
128 45.3561075089458
129 44.7465224950579
130 44.1505294634223
131 43.5679240342014
132 42.9984988382857
133 42.4420438618198
134 41.8983467818695
135 41.3671932930005
136 40.8483674245536
137 40.3416518484137
138 39.8468281770885
139 39.3636772519321
140 38.8919794213622
141 38.431514808944
142 37.9820635712337
143 37.5434061452911
144 37.1153234857991
145 36.6975972917451
146 36.2900102226427
147 35.8923461042957
148 35.5043901241268
149 35.125929016117
};
\addlegendentry{GD}
\addplot+[mark repeat=5]
table {%
0 240.383424498765
1 207.451365208832
2 179.697082387268
3 156.272100320735
4 136.496571408799
5 119.802235891656
6 105.688455849048
7 93.700242344613
8 83.4216469020899
9 74.4779566337852
10 66.5463489620443
11 59.374106932815
12 52.7951291486572
13 46.7304534818244
14 41.1667311777043
15 36.1219179720726
16 31.6142583993748
17 27.6445269476132
18 24.1916559424738
19 21.216615163031
20 18.6692868010566
21 16.4950871479489
22 14.6399938259687
23 13.0537772826316
24 11.69172935006
25 10.5153076497947
26 9.49207814857239
27 8.59525097091991
28 7.80301625140589
29 7.09781460864542
30 6.46562360242429
31 5.89530480373948
32 5.37803204835487
33 4.90680648109062
34 4.47605526575261
35 4.08130621181929
36 3.71892855451349
37 3.38592969642593
38 3.07979819766838
39 2.79838424960715
40 2.53981001050797
41 2.30240335512385
42 2.08464970097153
43 1.88515757399599
44 1.70263444615843
45 1.53587011491403
46 1.38372550697887
47 1.24512528860356
48 1.11905306618687
49 1.00454827912625
50 0.90070413517515
51 0.806666129792412
52 0.721630835999356
53 0.644844759489206
54 0.575603133019956
55 0.513248580949044
56 0.457169624400855
57 0.406799024215471
58 0.361611975851106
59 0.321124180412868
60 0.28488982097384
61 0.252499474877692
62 0.223577991919129
63 0.197782366045314
64 0.174799625128717
65 0.154344759871298
66 0.136158709317874
67 0.120006416985516
68 0.10567496838486
69 0.0929718177909326
70 0.0817231095502085
71 0.0717720969947594
72 0.0629776601628231
73 0.0552129219761642
74 0.0483639612699062
75 0.0423286200784768
76 0.0370154018196239
77 0.032342456455643
78 0.0282366483171396
79 0.0246327020228806
80 0.0214724217945804
81 0.0187039794262994
82 0.0162812662053245
83 0.0141633041786098
84 0.0123137123018589
85 0.010700223185495
86 0.00929424635300555
87 0.00807047414434145
88 0.00700652662359747
89 0.00608263208049077
90 0.00528133994517023
91 0.00458726316209303
92 0.00398684728860133
93 0.00346816379559007
94 0.00302072524977399
95 0.00263532024881688
96 0.00230386616127433
97 0.00201927789274583
98 0.00177535105781181
99 0.00156665808433271
100 0.00138845591287523
101 0.00123660407972442
102 0.00110749208763848
103 0.000997975074699259
104 0.000905316888844358
105 0.000827139764469396
106 0.000761379878464883
107 0.000706248136689364
108 0.000660195608754453
109 0.000621883089617886
110 0.000590154321328171
111 0.000564012457828851
112 0.000542599400439159
113 0.000525177671911569
114 0.000511114533200864
115 0.000499868079643832
116 0.000490975082468045
117 0.00048404036772826
118 0.000478727548222846
119 0.000474750944894969
120 0.000471868552955011
121 0.000469875924658952
122 0.000468600855570369
123 0.000467898774386414
124 0.00046764874819667
125 0.000467750025518378
126 0.000468119048748903
127 0.000468686875915246
128 0.000469396958906375
129 0.000470203231831485
130 0.000471068468862836
131 0.000471962875959783
132 0.000472862885330102
133 0.000473750125400691
134 0.000474610542525764
135 0.000475433653701456
136 0.000476211912224735
137 0.000476940170576522
138 0.00047761522687032
139 0.000478235443002992
140 0.000478800424225202
141 0.000479310751225513
142 0.000479767757025221
143 0.00048017334203276
144 0.000480529821519383
145 0.000480839800577455
146 0.000481106072311063
147 0.000481331535612993
148 0.000481519129402594
149 0.000481671780651221
};
\addlegendentry{NWT}

\end{groupplot}

\end{tikzpicture}




















% \nextgroupplot[
% axis line style={white!80!black},
% legend cell align={left},
% legend style={fill opacity=0.8, draw opacity=1, text opacity=1, at={(1,0.5)}, anchor=west, draw=none},
% log basis y={10},
% tick align=outside,
% tick pos=left,
% title={Error ||thetatrue - x\_i||},
% x grid style={white!80!black},
% xmajorgrids,
% xmin=-7.45, xmax=156.45,
% xtick style={color=white!15!black},
% xtick={-25,0,25,50,75,100,125,150,175},
% xticklabels={-20,0,20,40,60,80,100,120,140},
% y grid style={white!80!black},
% ymajorgrids,
% ymin=6.2115399106969e-05, ymax=2.20198887070396,
% ymode=log,
% ytick style={color=white!15!black},
% ytick={1e-06,1e-05,0.0001,0.001,0.01,0.1,1,10,100},
% yticklabels={\(\displaystyle 10^{-6}\),\(\displaystyle 10^{-5}\),\(\displaystyle 10^{-4}\),\(\displaystyle 10^{-3}\),\(\displaystyle 10^{-2}\),\(\displaystyle 10^{-1}\),\(\displaystyle 10^{0}\),\(\displaystyle 10^{1}\),\(\displaystyle 10^{2}\)}
% ]
% \addplot [ultra thick, color0]
% table {%
% 0 1.35648663834186
% 1 1.3605521791835
% 2 1.35553110190525
% 3 1.3588607863063
% 4 1.3627882368566
% 5 1.36777417532881
% 6 1.36777417532881
% 7 1.36777417532881
% 8 1.36777417532881
% 9 1.36101782987933
% 10 1.36101782987933
% 11 1.36101782987933
% 12 1.36101782987933
% 13 1.36101782987933
% 14 1.35666498911785
% 15 1.35666498911785
% 16 1.35666498911785
% 17 1.35283652296717
% 18 1.35283652296717
% 19 1.35324447892085
% 20 1.35324447892085
% 21 1.34875366443131
% 22 1.34875366443131
% 23 1.34875366443131
% 24 1.34875366443131
% 25 1.34875366443131
% 26 1.34875366443131
% 27 1.34875366443131
% 28 1.34897666678057
% 29 1.34672427155871
% 30 1.34506930898318
% 31 1.34506930898318
% 32 1.34506930898318
% 33 1.34506930898318
% 34 1.337017017985
% 35 1.32846533368326
% 36 1.32846533368326
% 37 1.32846533368326
% 38 1.32846533368326
% 39 1.32846533368326
% 40 1.32846533368326
% 41 1.32846533368326
% 42 1.32846533368326
% 43 1.32846533368326
% 44 1.32846533368326
% 45 1.32531049959485
% 46 1.32531049959485
% 47 1.32531049959485
% 48 1.32531049959485
% 49 1.32531049959485
% 50 1.32531049959485
% 51 1.33045337496353
% 52 1.33045337496353
% 53 1.32392647520326
% 54 1.32392647520326
% 55 1.32392647520326
% 56 1.3276252788285
% 57 1.3288631077686
% 58 1.3288631077686
% 59 1.3288631077686
% 60 1.3329944536256
% 61 1.3329944536256
% 62 1.3329944536256
% 63 1.33362249507783
% 64 1.33362249507783
% 65 1.33362249507783
% 66 1.33362249507783
% 67 1.33917190385722
% 68 1.3363967199562
% 69 1.3363967199562
% 70 1.3357285047428
% 71 1.3357285047428
% 72 1.33011938573639
% 73 1.33011938573639
% 74 1.33011938573639
% 75 1.33011938573639
% 76 1.32736408206047
% 77 1.32736408206047
% 78 1.32736408206047
% 79 1.32179309607081
% 80 1.32179309607081
% 81 1.32282245709677
% 82 1.32282245709677
% 83 1.32282245709677
% 84 1.32282245709677
% 85 1.32282245709677
% 86 1.32282245709677
% 87 1.31764419819261
% 88 1.31503360885886
% 89 1.31503360885886
% 90 1.31503360885886
% 91 1.31503360885886
% 92 1.31503360885886
% 93 1.31503360885886
% 94 1.31503360885886
% 95 1.31503360885886
% 96 1.31503360885886
% 97 1.31503360885886
% 98 1.31503360885886
% 99 1.31503360885886
% 100 1.31503360885886
% 101 1.30969828715458
% 102 1.30969828715458
% 103 1.30969828715458
% 104 1.31086939198843
% 105 1.31086939198843
% 106 1.31086939198843
% 107 1.30767105712827
% 108 1.30775123241381
% 109 1.3091188599801
% 110 1.31170139474989
% 111 1.30951959581183
% 112 1.31337716695491
% 113 1.31606120872614
% 114 1.31606120872614
% 115 1.30726243085938
% 116 1.30726243085938
% 117 1.30726243085938
% 118 1.30726243085938
% 119 1.30726243085938
% 120 1.30726243085938
% 121 1.30726243085938
% 122 1.30726243085938
% 123 1.30726243085938
% 124 1.30172093092616
% 125 1.30172093092616
% 126 1.29978102804401
% 127 1.2946787498389
% 128 1.2967680798809
% 129 1.290069655314
% 130 1.290069655314
% 131 1.290069655314
% 132 1.290069655314
% 133 1.28639140989148
% 134 1.27929849875297
% 135 1.27489768432954
% 136 1.27489768432954
% 137 1.27489768432954
% 138 1.27899786190205
% 139 1.27823400557149
% 140 1.27823400557149
% 141 1.27823400557149
% 142 1.27823400557149
% 143 1.27318568926819
% 144 1.27318568926819
% 145 1.27318568926819
% 146 1.27318568926819
% 147 1.27318568926819
% 148 1.27318568926819
% 149 1.27318568926819
% };
% \addlegendentry{Random Search}
% \addplot [ultra thick, color1]
% table {%
% 0 1.35648663834186
% 1 1.35207459252609
% 2 1.34747798200477
% 3 1.34265499800133
% 4 1.33769630753975
% 5 1.33274507715993
% 6 1.32782554401867
% 7 1.32293620637711
% 8 1.31807737298156
% 9 1.31324918457561
% 10 1.30845178017473
% 11 1.3036852839563
% 12 1.29894980609053
% 13 1.29424544262234
% 14 1.28957227547979
% 15 1.28493037254078
% 16 1.2803197877656
% 17 1.27574056139762
% 18 1.2711927202344
% 19 1.26667627797059
% 20 1.26219123561365
% 21 1.25773758197222
% 22 1.25331529421663
% 23 1.24892433850957
% 24 1.24456467070453
% 25 1.24023623710815
% 26 1.23593897530181
% 27 1.23167281501673
% 28 1.22743767905582
% 29 1.22323348425445
% 30 1.21906014247153
% 31 1.21491756160136
% 32 1.21080564659605
% 33 1.2067243004878
% 34 1.20267342539982
% 35 1.19865292353453
% 36 1.19466269812779
% 37 1.19070265435773
% 38 1.18677270019783
% 39 1.18287274720367
% 40 1.17900271122454
% 41 1.17516251303129
% 42 1.17135207885365
% 43 1.16757134082115
% 44 1.16382023730356
% 45 1.16009871314796
% 46 1.15640671981155
% 47 1.15274421539044
% 48 1.14911116454656
% 49 1.14550753833606
% 50 1.14193331394409
% 51 1.1383884743319
% 52 1.1348730078035
% 53 1.13138690749966
% 54 1.12793017082814
% 55 1.12450279883915
% 56 1.12110479555556
% 57 1.11773616726746
% 58 1.11439692180047
% 59 1.11108706776716
% 60 1.10780661381046
% 61 1.10455556784733
% 62 1.1013339363206
% 63 1.098141723466
% 64 1.09497893060071
% 65 1.0918455554391
% 66 1.08874159144038
% 67 1.08566702719218
% 68 1.08262184583338
% 69 1.07960602451863
% 70 1.07661953392641
% 71 1.07366233781189
% 72 1.07073439260517
% 73 1.06783564705498
% 74 1.06496604191756
% 75 1.06212550968995
% 76 1.05931397438652
% 77 1.0565313513576
% 78 1.05377754714837
% 79 1.05105245939654
% 80 1.04835597676665
% 81 1.04568797891929
% 82 1.04304833651304
% 83 1.04043691123718
% 84 1.03785355587308
% 85 1.03529811438228
% 86 1.0327704220193
% 87 1.0302703054672
% 88 1.02779758299413
% 89 1.02535206462897
% 90 1.02293355235447
% 91 1.02054184031624
% 92 1.01817671504594
% 93 1.01583795569741
% 94 1.01352533429419
% 95 1.01123861598724
% 96 1.00897755932155
% 97 1.00674191651062
% 98 1.00453143371752
% 99 1.00234585134177
% 100 1.00018490431085
% 101 0.998048322375541
% 102 0.995935830408298
% 103 0.993847148703707
% 104 0.991781993280404
% 105 0.989740076183659
% 106 0.987721105787975
% 107 0.985724787099053
% 108 0.983750822054518
% 109 0.981798909822817
% 110 0.979868747099748
% 111 0.97796002840211
% 112 0.976072446357949
% 113 0.974205691992971
% 114 0.972359455012652
% 115 0.970533424079633
% 116 0.968727287086007
% 117 0.96694073142013
% 118 0.9651734442276
% 119 0.963425112666073
% 120 0.96169542415363
% 121 0.959984066610402
% 122 0.958290728693187
% 123 0.956615100022846
% 124 0.954956871404238
% 125 0.953315735038526
% 126 0.95169138472767
% 127 0.950083516070967
% 128 0.948491826653513
% 129 0.946916016226489
% 130 0.945355786879179
% 131 0.943810843202675
% 132 0.942280892445228
% 133 0.940765644659213
% 134 0.939264812839744
% 135 0.937778113054921
% 136 0.936305264567787
% 137 0.934845989950038
% 138 0.933400015187566
% 139 0.931967069777931
% 140 0.930546886819881
% 141 0.929139203095037
% 142 0.927743759141888
% 143 0.926360299322257
% 144 0.924988571880397
% 145 0.923628328994899
% 146 0.922279326823607
% 147 0.920941325541728
% 148 0.919614089373364
% 149 0.918297386616658
% };
% \addlegendentry{GD}
% \addplot [ultra thick, color2]
% table {%
% 0 1.35648663834186
% 1 1.10927157537186
% 2 0.91355487167021
% 3 0.75785444328672
% 4 0.633458437812904
% 5 0.533726921061318
% 6 0.453592164868818
% 7 0.389181996207227
% 8 0.337525501479084
% 9 0.29631955485996
% 10 0.263745013152772
% 11 0.238325921911076
% 12 0.218826064656193
% 13 0.204177120578757
% 14 0.193433912301885
% 15 0.185753215673202
% 16 0.180390451212139
% 17 0.176705078761817
% 18 0.17416523897597
% 19 0.172346050680886
% 20 0.170920861663561
% 21 0.169647770178343
% 22 0.168354402639676
% 23 0.166923238478071
% 24 0.165278749576927
% 25 0.163376800865393
% 26 0.161196262361503
% 27 0.158732549342565
% 28 0.155992737206098
% 29 0.152991911742812
% 30 0.149750464352251
% 31 0.146292098604445
% 32 0.142642367249013
% 33 0.138827602882374
% 34 0.134874140394393
% 35 0.130807756016153
% 36 0.126653267761811
% 37 0.122434256772901
% 38 0.118172879806096
% 39 0.113889750881275
% 40 0.109603875719781
% 41 0.10533262665145
% 42 0.101091748596423
% 43 0.096895388857004
% 44 0.0927561450189488
% 45 0.0886851264268224
% 46 0.0846920255817382
% 47 0.0807851964940562
% 48 0.0769717375653413
% 49 0.0732575770121953
% 50 0.0696475592062048
% 51 0.0661455306074205
% 52 0.0627544242259352
% 53 0.0594763417658762
% 54 0.0563126327945513
% 55 0.0532639704410341
% 56 0.0503304232665744
% 57 0.0475115230666253
% 58 0.0448063284633355
% 59 0.0422134842301462
% 60 0.0397312763585192
% 61 0.0373576829325607
% 62 0.0350904209219884
% 63 0.032926989039029
% 64 0.0308647068318165
% 65 0.0289007502069833
% 66 0.0270321835885892
% 67 0.0252559889304414
% 68 0.0235690918052547
% 69 0.0219683847979824
% 70 0.0204507484329853
% 71 0.0190130698664806
% 72 0.01765225957796
% 73 0.0163652662981612
% 74 0.015149090418086
% 75 0.014000796135204
% 76 0.0129175226115593
% 77 0.0118964944469673
% 78 0.0109350318128177
% 79 0.0100305606536821
% 80 0.00918062345241505
% 81 0.00838289117989059
% 82 0.00763517722625964
% 83 0.00693545435314151
% 84 0.00628187603325091
% 85 0.00567280396762579
% 86 0.00510684407764973
% 87 0.004582893772301
% 88 0.00410020351647599
% 89 0.00365845496832057
% 90 0.00325785459548354
% 91 0.00289923241674615
% 92 0.00258411467054723
% 93 0.00231470032622624
% 94 0.0020936173997189
% 95 0.00192330580442839
% 96 0.00180497316688628
% 97 0.00173739555381806
% 98 0.00171621693588368
% 99 0.00173432523769814
% 100 0.00178317423615236
% 101 0.00185429045966096
% 102 0.00194030067678119
% 103 0.00203532901180694
% 104 0.00213495740274425
% 105 0.00223599083549667
% 106 0.0023361835368291
% 107 0.00243399613515184
% 108 0.00252840332517284
% 109 0.00261874963320053
% 110 0.00270464409973836
% 111 0.00278588427664309
% 112 0.00286240156947905
% 113 0.00293422188846997
% 114 0.00300143722484106
% 115 0.00306418503142515
% 116 0.00312263320160351
% 117 0.00317696908845141
% 118 0.0032273914597856
% 119 0.00327410460194939
% 120 0.00331731400724984
% 121 0.00335722323622551
% 122 0.0033940316565872
% 123 0.00342793283963193
% 124 0.00345911345171182
% 125 0.00348775251951068
% 126 0.00351402097797381
% 127 0.00353808143191243
% 128 0.00356008807877569
% 129 0.00358018675240513
% 130 0.00359851505688005
% 131 0.00361520256660846
% 132 0.0036303710742095
% 133 0.00364413487186864
% 134 0.00365660105504986
% 135 0.00366786983993396
% 136 0.00367803488789306
% 137 0.0036871836318349
% 138 0.00369539760044595
% 139 0.00370275273730848
% 140 0.00370931971261645
% 141 0.00371516422580601
% 142 0.00372034729788815
% 143 0.0037249255526459
% 144 0.00372895148615419
% 145 0.00373247372431444
% 146 0.00373553726828404
% 147 0.00373818372782378
% 148 0.00374045154270157
% 149 0.00374237619237911
% };
% \addlegendentry{Newton}
% \addplot [ultra thick, red!54.5098039215686!black, dashed]
% table {%
% 0 0.136845509446949
% 1 0.136845509446949
% 2 0.136845509446949
% 3 0.136845509446949
% 4 0.136845509446949
% 5 0.136845509446949
% 6 0.136845509446949
% 7 0.136845509446949
% 8 0.136845509446949
% 9 0.136845509446949
% 10 0.136845509446949
% 11 0.136845509446949
% 12 0.136845509446949
% 13 0.136845509446949
% 14 0.136845509446949
% 15 0.136845509446949
% 16 0.136845509446949
% 17 0.136845509446949
% 18 0.136845509446949
% 19 0.136845509446949
% 20 0.136845509446949
% 21 0.136845509446949
% 22 0.136845509446949
% 23 0.136845509446949
% 24 0.136845509446949
% 25 0.136845509446949
% 26 0.136845509446949
% 27 0.136845509446949
% 28 0.136845509446949
% 29 0.136845509446949
% 30 0.136845509446949
% 31 0.136845509446949
% 32 0.136845509446949
% 33 0.136845509446949
% 34 0.136845509446949
% 35 0.136845509446949
% 36 0.136845509446949
% 37 0.136845509446949
% 38 0.136845509446949
% 39 0.136845509446949
% 40 0.136845509446949
% 41 0.136845509446949
% 42 0.136845509446949
% 43 0.136845509446949
% 44 0.136845509446949
% 45 0.136845509446949
% 46 0.136845509446949
% 47 0.136845509446949
% 48 0.136845509446949
% 49 0.136845509446949
% 50 0.136845509446949
% 51 0.136845509446949
% 52 0.136845509446949
% 53 0.136845509446949
% 54 0.136845509446949
% 55 0.136845509446949
% 56 0.136845509446949
% 57 0.136845509446949
% 58 0.136845509446949
% 59 0.136845509446949
% 60 0.136845509446949
% 61 0.136845509446949
% 62 0.136845509446949
% 63 0.136845509446949
% 64 0.136845509446949
% 65 0.136845509446949
% 66 0.136845509446949
% 67 0.136845509446949
% 68 0.136845509446949
% 69 0.136845509446949
% 70 0.136845509446949
% 71 0.136845509446949
% 72 0.136845509446949
% 73 0.136845509446949
% 74 0.136845509446949
% 75 0.136845509446949
% 76 0.136845509446949
% 77 0.136845509446949
% 78 0.136845509446949
% 79 0.136845509446949
% 80 0.136845509446949
% 81 0.136845509446949
% 82 0.136845509446949
% 83 0.136845509446949
% 84 0.136845509446949
% 85 0.136845509446949
% 86 0.136845509446949
% 87 0.136845509446949
% 88 0.136845509446949
% 89 0.136845509446949
% 90 0.136845509446949
% 91 0.136845509446949
% 92 0.136845509446949
% 93 0.136845509446949
% 94 0.136845509446949
% 95 0.136845509446949
% 96 0.136845509446949
% 97 0.136845509446949
% 98 0.136845509446949
% 99 0.136845509446949
% 100 0.136845509446949
% 101 0.136845509446949
% 102 0.136845509446949
% 103 0.136845509446949
% 104 0.136845509446949
% 105 0.136845509446949
% 106 0.136845509446949
% 107 0.136845509446949
% 108 0.136845509446949
% 109 0.136845509446949
% 110 0.136845509446949
% 111 0.136845509446949
% 112 0.136845509446949
% 113 0.136845509446949
% 114 0.136845509446949
% 115 0.136845509446949
% 116 0.136845509446949
% 117 0.136845509446949
% 118 0.136845509446949
% 119 0.136845509446949
% 120 0.136845509446949
% 121 0.136845509446949
% 122 0.136845509446949
% 123 0.136845509446949
% 124 0.136845509446949
% 125 0.136845509446949
% 126 0.136845509446949
% 127 0.136845509446949
% 128 0.136845509446949
% 129 0.136845509446949
% 130 0.136845509446949
% 131 0.136845509446949
% 132 0.136845509446949
% 133 0.136845509446949
% 134 0.136845509446949
% 135 0.136845509446949
% 136 0.136845509446949
% 137 0.136845509446949
% 138 0.136845509446949
% 139 0.136845509446949
% 140 0.136845509446949
% 141 0.136845509446949
% 142 0.136845509446949
% 143 0.136845509446949
% 144 0.136845509446949
% 145 0.136845509446949
% 146 0.136845509446949
% 147 0.136845509446949
% 148 0.136845509446949
% 149 0.136845509446949
% };
% \addlegendentry{InvProb noise WITH Solver-Unc. (1.4e-01)}
% \addplot [ultra thick, white!50.1960784313725!black, dotted]
% table {%
% 0 0.0001
% 1 0.0001
% 2 0.0001
% 3 0.0001
% 4 0.0001
% 5 0.0001
% 6 0.0001
% 7 0.0001
% 8 0.0001
% 9 0.0001
% 10 0.0001
% 11 0.0001
% 12 0.0001
% 13 0.0001
% 14 0.0001
% 15 0.0001
% 16 0.0001
% 17 0.0001
% 18 0.0001
% 19 0.0001
% 20 0.0001
% 21 0.0001
% 22 0.0001
% 23 0.0001
% 24 0.0001
% 25 0.0001
% 26 0.0001
% 27 0.0001
% 28 0.0001
% 29 0.0001
% 30 0.0001
% 31 0.0001
% 32 0.0001
% 33 0.0001
% 34 0.0001
% 35 0.0001
% 36 0.0001
% 37 0.0001
% 38 0.0001
% 39 0.0001
% 40 0.0001
% 41 0.0001
% 42 0.0001
% 43 0.0001
% 44 0.0001
% 45 0.0001
% 46 0.0001
% 47 0.0001
% 48 0.0001
% 49 0.0001
% 50 0.0001
% 51 0.0001
% 52 0.0001
% 53 0.0001
% 54 0.0001
% 55 0.0001
% 56 0.0001
% 57 0.0001
% 58 0.0001
% 59 0.0001
% 60 0.0001
% 61 0.0001
% 62 0.0001
% 63 0.0001
% 64 0.0001
% 65 0.0001
% 66 0.0001
% 67 0.0001
% 68 0.0001
% 69 0.0001
% 70 0.0001
% 71 0.0001
% 72 0.0001
% 73 0.0001
% 74 0.0001
% 75 0.0001
% 76 0.0001
% 77 0.0001
% 78 0.0001
% 79 0.0001
% 80 0.0001
% 81 0.0001
% 82 0.0001
% 83 0.0001
% 84 0.0001
% 85 0.0001
% 86 0.0001
% 87 0.0001
% 88 0.0001
% 89 0.0001
% 90 0.0001
% 91 0.0001
% 92 0.0001
% 93 0.0001
% 94 0.0001
% 95 0.0001
% 96 0.0001
% 97 0.0001
% 98 0.0001
% 99 0.0001
% 100 0.0001
% 101 0.0001
% 102 0.0001
% 103 0.0001
% 104 0.0001
% 105 0.0001
% 106 0.0001
% 107 0.0001
% 108 0.0001
% 109 0.0001
% 110 0.0001
% 111 0.0001
% 112 0.0001
% 113 0.0001
% 114 0.0001
% 115 0.0001
% 116 0.0001
% 117 0.0001
% 118 0.0001
% 119 0.0001
% 120 0.0001
% 121 0.0001
% 122 0.0001
% 123 0.0001
% 124 0.0001
% 125 0.0001
% 126 0.0001
% 127 0.0001
% 128 0.0001
% 129 0.0001
% 130 0.0001
% 131 0.0001
% 132 0.0001
% 133 0.0001
% 134 0.0001
% 135 0.0001
% 136 0.0001
% 137 0.0001
% 138 0.0001
% 139 0.0001
% 140 0.0001
% 141 0.0001
% 142 0.0001
% 143 0.0001
% 144 0.0001
% 145 0.0001
% 146 0.0001
% 147 0.0001
% 148 0.0001
% 149 0.0001
% };
% \addlegendentry{InvProb noise (1.0e-04)}

